Answer Them All! Toward Universal Visual Question Answering Models

Visual Question Answering (VQA) research is split into two camps: the first focuses on VQA datasets that require natural image understanding and the second focuses on synthetic datasets that test reasoning. A good VQA algorithm should be capable of both, but only a few VQA algorithms are tested in this manner. We compare five state-of-the-art VQA algorithms across eight VQA datasets covering both domains. To make the comparison fair, all of the models are standardized as much as possible, e.g., they use the same visual features, answer vocabularies, etc. We find that methods do not generalize across the two domains. To address this problem, we propose a new VQA algorithm that rivals or exceeds the state-of-the-art for both domains.

==> oldText.tex <==

\cleardoublepage


\section{\kk{EVERYTHING THAT WAS HERE BEFORE I MADE A NEW STRUCTURE. A LOT CAN BE COPIED OVER BUT WANTED A CLEAN SLATE THAT WE CAN ALL COMMENT ON}}
\section{\rs{We can copy some sections from my deep Learning draft: 
}}
\url{https://www.overleaf.com/1551332779pgwvcbpwptgn}


%%%%%%%%% ABSTRACT
\section{OLD CONTENT}
\begin{abstract}
    Current Visual Question Answering (VQA) research has been split into two camps: the first focuses on natural VQA datasets that require natural image understanding, while the second focuses on synthetic datasets to test compositional reasoning skills. There are other VQA datasets testing generalization power of VQA methods, but current methods rarely evaluate on them. This defeats the purpose behind creating these datasets, which was to showcase methods that can understand real-world visuo-linguistic concepts and perform reasoning. It is not clear what these VQA methods are exactly capable of, so to gauge true capability of these VQA models we evaluate five state-of-the-art VQA algorithms by passing them through a gauntlet of tests. We use \gls{VQAv1} and VQAv2 to test natural image understanding, \cvqa~to evaluate performance under unseen concept compositions and \vqacp~to analyze generalization to different answer distributions. We examine task generalization and identify difficult question types using TDIUC. We use CLEVR and CLEVR-Humans to test compositional reasoning skills and CoGenT to examine if models are able to compose concepts in novel manner and remember old concepts. Our work demonstrates that many methods that work well on one dataset fail on the rest, illustrating the need for single model that works well across datasets. Taking a bold step towards that goal, we propose a new model Bilinear Attentional Reasoning Network (BARN) that is capable of both natural image understanding and compositional reasoning, and will hopefully show equal or better performance on all generalization tests.
\end{abstract}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\textwidth]{images/main-problem.jpg}
    \caption{Main Diagram showing our major point. Something like this is fine, but hopefully something a bit punchier.}
    \label{fig:main-problem}
\end{figure}

\section{Introduction}
Visual Question Answering (VQA) requires agents to understand visuo-linguistic concepts and perform reasoning to answer questions about visual content. For example, natural VQA datasets\rs{CITE} ask questions requiring real-world scene understanding, object recognition and activity recognition among other abilities to predict answers. However, instead of learning and reasoning with concepts models that simply exploit dataset biases can achieve good performances on such datasets\rs{CITE}.

To address this issue, several natural-image VQA datasets were introduced where models cannot simply exploit statistical biases to answer questions\rs{CITE}. For instance, by using a test answer distribution that is completely different from train dataset, VQACP\rs{CITE} ensures that models which simply memorize correlations in training dataset fail during test. Another diagnostic dataset: CLEVR\rs{CITE} tests compositional reasoning abilities such as: counting and logical reasoning to answer questions about synthetic images. VQA community has access to all these diagnostic datasets that can reveal a lot about VQA models. However, new VQA models are usually either evaluated only on VQAv2, where it is still possible to exploit biases or only on CLEVR, which does not require natural image understanding. Therefore, it is not clear what VQA models are truly capable of achieving.% all of these requirements, because they are evaluated against only specific datasets that they are designed for. VQA models that have focused on attentive fusion mechanisms to connect language with vision have been achieving state-of-the-art results on natural VQA datasets~\cite{anderson2017bottom,fukui2016multimodal,kim2018bilinear,lu2016hierarchical,norcliffe2018learning}. However, these works do not report results on datasets requiring compositional reasoning. A separate camp of VQA algorithms focus on compositional reasoning using modular~\cite{} or non-modular approaches~\cite{}, however these algorithms have not been evaluated on natural VQA datasets. So, it is not clear if their reasoning skills generalize to natural concepts. skills~\cite{johnson2017inferring, andreas2016neural, hu2017learning,mascharka2018transparency}. There are other natural VQA datasets that perform generalization tests: TDIUC tests generalization to multiple tasks, CVQA examines if algorithms are able to compose known concepts in novel ways and VQACP tests the generalization to unknown answer distributions. Current works do not report their results on these datasets, so it is unclear how well the models generalize.

In this work, we choose five representative state-of-the-art VQA models and evaluate them on all major VQA datasets to examine their true abilities. We test natural concept understanding with VQAv1 and VQAv2. We evaluate the ability to combine seen concepts in previously unseen ways using CVQA\rs{CITE}. We test generalization to unknown answer distributions using VQACP\rs{CITE}. We use the Task Driven Understanding Challenge (TDIUC)\rs{CITE} to determine generalization to different tasks and examine the question types that still trouble current methods. We evaluate compositional reasoning skills using Compositional Language and Elementary Visual Reasoning (CLEVR) dataset and use their generalization task: CLEVR-CoGenT to test the ability to handle unseen concept combinations and remember old concepts. Our comprehensive tests show that none of the current algorithms perform well across all datasets, illustrating the need for single model that shows concept understanding, reasoning and generalization.
%Our comprehensive evaluation identifies several problems with current VQA models. VQA algorithms that achieve state-of-the-art results on natural VQA datasets, fail on compositional reasoning datasets and VQA algorithms capable of compositional reasoning fail on natural VQA datasets. All VQA algorithms struggle to generalize to multiple tasks, work with unknown concept compositions or handle unknown distributions, illustrating that significant work is required to create VQA models with all these capabilities. To this end, we propose a model that we believe will work well on all kinds of datasets.

We propose a new VQA model: Bilinear Attentional Relation Network (BARN), that combines visual and question information in a way that enables both natural image understanding and compositional reasoning, hopefully showing near state-of-the-art or even improved performance across all datasets. %The proposed model: Bilinear Attention over Bimodal Embeddings (BABE), first applies early fusion on visual and question features, which is known to enable compositional reasoning\rs{CITE}. The early fusion generates Bimodal Embeddings, which are passed through a bilinear attention mechanism\rs{CITE} to predict multi-glimpse bilinear attention maps. These maps weights bimodal embedding pairs by their relevance to the VQA task. The maps are used to capture bilinear interactions between the bimodal embeddings, generating the BABE vector which encodes question relevant scene features. This embedding encodes all the visual-linguistic information required to answer the questions.


%multi-modal interactions between visual, textual and relational information to excel on both natural image understanding and synthetic compositional reasoning tasks. We hypothesize that current natural VQA models lack compositional reasoning because they do not capture relations between visual elements which are necessary to answer questions that involve integrating information from multiple visual objects. We further hypothesize that, relation networks that do explicitly capture relations between visual objects~\cite{santoro2017simple, desta2018object}, use inadequate strategies to fuse those relations with textual features (e.g., simple concatenation ~\cite{desta2018object}), which weakens their performance. The performance is further limited because they discard object features after capturing relations.

%In contrast, we predict answers using all pieces of information: object features, relation features, object-question interactions and relation-question interactions. Specifically, we use bilinear attention mechanism~\cite{kim2018bilinear} which weights visual and relational features by their relevance to the question and captures interactions between every relevant object/relation with question to produce an answer. We propose two alternate strategies to capture such interactions: in the first strategy, we use separate bilinear attention maps: a) to combine visual objects with text and b) to combine relations with text. In the second strategy, we combine object pairs and their relations before applying bilinear attention mechanism to fuse with text. We evaluate both alternatives on VQA2.0 and CLEVR. If the  models perform well on both kinds of datasets, we will further perform generalization tests on Task Driven Image Understanding Challenge (TDIUC)~\cite{kafle2017analysis}, Compositional VQA (C-VQA)~\cite{agrawal2017c}, VQA under Changing Priors (VQA-CP)~\cite{agrawal2018don}, CLEVR-Co Generalization Tests (CoGenT) and CLEVR-Humans~\cite{johnson2017clevr}.


We make the following  contributions:
\begin{itemize}
    \item We perform an extremely thorough comparison of five state-of-the-art VQA algorithms on a range of datasets, testing natural image understanding, reasoning skills and generalization abilities. None of the earlier works have reported results on all of these VQA tasks.
    
    \item To make the comparisons fair, we feed in same visual features to all models. This involved modifying existing architectures to be compatible with same input.
    
    \item Our experiments reveal major problems with current VQA models: 1) methods that work on natural VQA datasets fail when asked to perform reasoning and models with compositional reasoning fail on natural images. 2) All of the models lack generalization to multiple task types, new concept compositions and new answer distributions
    
    \item We present a new model that is capable of both natural image understanding and compositional reasoning, hopefully showing equal/improved performance on all of the challenging generalization tests.
\end{itemize}

This project was a huge undertaking, that required modifying and optimizing many VQA algorithms, consuming over 3000 GPU hours.

\section{Related Work}
\rs{TODO}
Visual Question Answering has gathered a lot of interest from both computer vision and natural language processing communities. In recent years, many algorithms\rs{CITEMANY} and datasets\rs{CITEMANY} have been released to address VQA. Attentive fusion mechanisms~\cite{anderson2017bottom,lu2016hierarchical,nam2016dual,fukui2016multimodal,ben2017mutan} have been the major focus of natural VQA algorithms. Attention computes relevance scores over visual and textual features allowing to models to process only relevant information and fusion mechanisms capture rich interactions between visual and textual modalities. 

However, such models are known exploit dataset biases instead of learning to understand and reason with visual concepts. So, researchers released more challenging VQA datasets\rs{CITE} that analyze the generalization capabilities of VQA models. Many VQA algorithms fail on these datasets because they can no longer exploit statistical correlations to predict answers. Unfortunately, current VQA methods do report results on these generalization tests. In this work, we evaluate algorithms on all of these datasets to gauge their true capability.

Next, CLEVR\rs{CITE} dataset was introduced to test reasoning skills, showing that the then natural-image based VQA algorithms lacked reasoning skills. Now, VQA research has come up with algorithms that achieve 99\% accuracy on this dataset\rs{CITEMANY}. Such algorithms either used pre-defined modules\rs{CITE} each primed to perform specific reasoning task or learn reasoning functions from data\rs{CITE}. However such methods are very rarely evaluated on natural-image based VQA datasets, so it is unclear if their reasoning skills generalize to natural images. In this paper, we evaluate compositional algorithms on natural datasets too.

%Through extensive experimentation involving XXX algorithms and XXX different datasets, and a lot of efforts of bringing all algorithms to the same page (by upgrading/using same features etc) we show that the algorithms do not transfer over to other algoirthms. Acknowledge that CLEVR paper already shows some of this as it shows VQA algorithms such as SAN dont work well. But we further show that even more modern algorithms are very poor on clevr. Similarly, newer algoirithms that are designed for compositional reasoning on clevr do not perform well even when the features are appropriately upgraded. 

%Finally, say that contrary to prior work our algorithm which tackles trying to address real-world challenges posed by VQA and its variants as well as additional challenges posed by diagnostic datasets such as CLEVR, CoGENT etc..}


\section{Part I: How well do algorithms perform across natural and synthetic datasets?}
To examine the generalizability of current VQA models to different VQA tasks, we choose five representative state-of-the-art VQA methods and run them on eight challenging VQA datasets.
\subsection{Tested Algorithms}
\textbf{Bottom-Up-Attention and Top-Down (\gls{UpDn})}~\cite{anderson2017bottom} combines bottom-up and top-down attention mechanisms to perform VQA, with bottom-up mechanism generating object proposals from Faster-RCNN~\cite{ren2015faster}, and the top-down mechanism predicting an attention distribution over those proposals. The top-down attention is task-driven, using questions to predict attention weights over the image regions. This model obtained first place in the 2017 VQA Challenge. For fair comparison, we use bottom-up object features as used in this work for all other VQA models.

\textbf{Question-Conditioned Graph (\qcg)}~\cite{norcliffe2018learning} represents images as graphs where object-level features from bottom-up object proposals\rs{CITE} act as graph nodes and edges that encode interactions between the objects are conditioned on the question. For each node, QC-Graph chooses a neighborhood of nodes with strongest edge connections, resulting in a question specific graph structure. This structure is processed by a patch operator to perform spatial graph convolution\rs{CITE}. The  main reason for choosing this model was to examine if the presented graph convolutions were capable of capturing object/object interactions required for compositional reasoning.

\textbf{Bilinear Attention Networks (BAN)}\rs{CITE} fuses visual and textual modalities by considering interactions between all visual objects (visual channels) with all question words (textual channels). BAN is different from dual-attention mechanisms\cite{} because it handles interactions between all channels apart from just computing attention. It is a more general form of low-rank bilinear pooling methods that jointly represent each channel pair \rs{READ+CITE coattention, low rank pooling}. BAN supports multiple glimpses of attention connected via residual connections. It reports a score of 70.35\% on test-std split of \gls{VQAv2}, which is the current state-of-the-art on \gls{VQAv2} \rs{(need to verify this)}.

\textbf{Relation Network (\gls{RN})}~\cite{santoro2017simple} presents a simple yet very powerful reasoning mechanism. It pairs up objects, embeds the object pairs and sums them up. The sum is a vector that encodes question relevant relational information required for reasoning, as demonstrated by the performance on CLEVR. However, RN's computation complexity increases quadratically with the number of objects, making it expensive to run when the number of objects is large. In \rs{CITE}, the authors used a hard attention mechanism to select only a few objects to send to relation network. However, hard attention mechanisms are non-differentiable and difficult to learn\rs{CITE}. In this work, we utilize an even simpler, and yet more effective reasoning mechanism without pairing up objects or using hard attention.

\textbf{Memory, Attention and Composition \gls{MAC}} network~\cite{hudson2018compositional} presents computational cells which automatically learn to perform attention-based reasoning. Unlike, the modular networks\rs{CITE} that require pre-defined modules to perform pre-specified reasoning functions, MAC learns reasoning mechanisms directly from the data. Each MAC cell maintains a control state representing reasoning operation and a memory state that is the result of the reasoning operation. Each cell consists of: 1) a control unit that updates the control state 2) a read unit that extracts information from image representation and, 3) a write unit that updates its memory state which is later used to predict the answer. Their paper reports significant improvements on counting and numerical comparison tasks, which are the most challenging CLEVR tasks.

\subsection{Tested Datasets}
\textbf{\gls{VQAv1}/\gls{VQAv2}} \gls{VQAv1}\rs{CITE} is an open-ended visual question answering dataset consisting of over 248K train, 121K val and 244K test question/image pairs. \gls{VQAv2}~\cite{goyal2017making} is its newer version that addresses language bias by collecting complementary images resulting in different answers for same question. It consists of over 443K train, 214K val and 453 test question/image pairs. Both datasets contain questions requiring scene understanding, object/attribute/activity recognition and reasoning skills such as: counting and spatial reasoning, but they do not annotate questions with such nuanced question types.

%\subsection{TDIUC for nuanced task understanding}
\textbf{\gls{TDIUC}} ~\cite{kafle2017analysis} provides nuanced question types to test task understanding. The dataset consists of 12 task types: ``object presence'', ``scene classification'', ``sports recognition'', ``activity recognition'', ``counting'', ``positional reasoning'', ``sentiment understanding'', ``color attributes'', ``utility'', ``subordinate object recognition'', ``other attributes'' and ``absurd questions'' for 1.6M+ question answer pairs. 

%\subsection{C-VQA to test generalization to unseen natural concept compositions}
\textbf{\gls{CVQA}}~\cite{agrawal2017c} is a split of \gls{VQAv1} where test split consists of concept combinations that are not present in the train set. For \eg if the train set asks about ``green plate'' and ``red light'', the test set will ask about ``red plate'' and ``green light''. This tests the ability to combine previously seen concepts in previously unseen combinations.

% For e.g., if the test set contains question answer pairs such as: (Q: ``What $\textbf{color}$ is the $\textbf{stop light}$?'', A: ``$\textbf{Green}$'') and (Q: ``What is the $\textbf{color}$ of the $\textbf{plate}$?'',  A: ``$\textbf{Red}$''), then the train set does not contain question answer pairs containing those concept combinations i.e., (``color'', ``stop light'', ``green'') or (``color'', ``plate'', ``red''). The train set however, does have question answer pairs where the individual concepts occur independently such as: (Q: ``What $\textbf{color}$ is the $\textbf{plate}$?'', A: ``$\textbf{Green}$'') and (Q: ``What $\textbf{color}$ are the $\textbf{stop lights}$?'', A: ``$\textbf{Red}$''). The reported results showed significant drop in performance for non-compositional VQA models~\cite{} and smaller but still significant drop for compositional models~\cite{}, indicating inability of VQA models to combine concepts. \rs{num. qns etc}

%\subsection{VQA-CP to test generalization to new distributions}
%Visual Question Answering under Changing Priors 
\textbf{\gls{VQACPv1}}\rs{CITE} re-organizes \gls{VQAv1} dataset so that answers for each question type are distributed differently in the train and test splits. This makes it very difficult for models that simply memorize training correlations to perform well on test set. For \eg ``blue'' and ``white'' might be the most frequent answers to ``What color'' questions in train set, but will rarely occur in the test set, making it impossible for algorithms perform well by exploiting such biases.

%\subsection{CLEVR/CLEVR-Humans to test Compositional Reasoning}
%Compositional Language and Elementary Visual Reasoning (CLEVR)~\cite{johnson2017clevr} 

\textbf{\gls{CLEVR}}~\cite{johnson2017clevr} provides simple synthetic scenes with 700K train, 15K val and 15K test questions requiring long chains of complex compositional reasoning skills. Answering CLEVR questions requires comparing attributes, performing spatial reasoning, remembering previously computed steps to predict the answer. It categorizes question types into: ``querying attribute'', ``comparing attributes'', ``existence'', ``counting'' and ``integer comparisons'', enabling diagnosis of specific reasoning abilities.

\textbf{\gls{CLEVR-Humans}}\rs{CITE: IEP} provides human-based questions for CLEVR scenes. It contains over 17.5K train, 7.2K val and 7.1K test questions, testing generalization to free-form questions.

%\subsection{CLEVR-CoGenT to test Generalization and Forgetting} 

\textbf{\gls{CoGenT}} contains two splits: A and B, arranged such that shape+color combinations are mutually exclusive in train and test sets (except for ``spehere''). If a model trained only on split A performs well on B too, then it implies the model has learned to combine concepts without being trained on those combinations. If a model first trained on split A and then fine-tuned on B still performs well on A, then it implies that the model has not forgotten to reason about old concept combinations even though it hasn't revisited them for a while.


\begin{table*}[!htbp]
\centering
\begin{tabular}{l|rrrrrr}
\hline
 Dataset/Algorithm & \multicolumn{1}{l}{UpDn} & \multicolumn{1}{l}{\qcg} & \multicolumn{1}{l}{BAN} & \multicolumn{1}{l}{MAC} & \multicolumn{1}{l}{RN} & \multicolumn{1}{l}{BARN} \\ \hline
VQA1 & 66.80 & 60.58 & \textbf{71.48} & 63.88 & 54.35 &  \\ VQA2 & 64.53 & 65.35 & \textbf{69.24} & 54.70 & 61.34 &  \\ \hline
TDIUC & 82.91 & 82.05 & \textbf{84.81} & 82.53 &  &  \\ C-VQA & 60.94 & 60.67 & \textbf{63.4} & 43.56 & 58.93 &  \\ VQA-CP & 39.77 & 37.86 & \textbf{42.04} & 33.86 & 36.30 &  \\ \hline
CLEVR & 65.86 & 43.51 & 75.56 & \textbf{98.00} & 95.97 &  \\
CLEVR-Humans (Before FT) & 54.51 & 28.41 & \textbf{61.03} & 50.20 & 57.65 &  \\
CLEVR-Humans (After FT) & 65.35 & 35.16 & 61.09 & \textbf{68.90} & 63.95 &  \\ \hline
CLEVR-CoGenT-A & 63.50 & 48.13 & 70.44 & \textbf{90.40} & 84.68 &  \\
CLEVR-CoGenT-B
(Before FT) & 68.07 & 52.47 & 77.44 & \textbf{98.04} & 96.09 &  \\
CLEVR-CoGenT-B
(After FT) & 65.95 & 46.97 & 76.75 & \textbf{97.20} & 96.45 &  \\
CLEVR-CoGenT-A
(After FT) & 67.96 & 51.81 & 74.12 & \textbf{98.45} & 97.44 &  \\ \end{tabular}
\caption{Comparison of VQA models on natural and synthetic datasets. Natural algorithms (UpDn, \qcg, BAN) fail on CLEVR, whereas MAC and RN show subpar performance on natural VQA Dataset.}
\label{tbl:all_vs_all}
\end{table*}


\subsection{Problems with current algorithms}
As shown in \tbl~\ref{tbl:all_vs_all}, none of the current VQA models work well on all datasets. Algorithms designed for natural images fail on compositional reasoning tasks and methods with reasoning skills fail on natural images. Results on \gls{TDIUC} shows algorithms lack task generalization. As indicated by performance on \gls{CVQA}, all of the algorithms show performance drop when asked to compose new concepts. \gls{VQACPv1} shows that algorithms completely fail when answer distribution changes.
\rs{TODO}


\section{Part II: Designing an algorithm that works well across datasets}
We identify the key strengths of existing algorithms that make them work and use them to devise a new model that will hopefully work well across all datasets. 

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{images/babe.png}
    \caption{Bilinear Attentional Reasoning Network (BARN) model, first concatenates object features (Obj) with question features (Q) and passes them through linear projections, generating bimodal embeddings (E). The model then predicts a bilinear attention map between embeddings. The model uses the attention map to capture interactions, resulting in BARN vector. This vector is fed into an MLP to predict the answer.}
    \label{fig:babe}
\end{figure*}

\subsection{Bilinear Attentional Reasoning Network (BARN)}
BARN uses early fusion between visual and textual features, which is known to enable compositional reasoning\rs{CITE}, and then captures interactions between the fused, bimodal embeddings using bilinear attention mechanism\rs{CITE} to predict the answer. In \rs{CITE}, the authors generated similar embeddings by concatenating question feature with CNN features (which was also trained end-to-end). They found that simply sum-pooling such embeddings and feeding them into an answer classifier, achieves impressive performance on CLEVR. However, they have not evaluated the approach on other VQA datasets. When we used similar approach with bottom-up features on \gls{VQAv2}, we found that ....\rs{hopefully won't as well as our new approach} To improve natural image understanding, our approach captures bilinear interactions between these embeddings instead of simply summing them up. BARN first predicts a bilinear attention map that encodes relevance of these embeddings for the VQA task and then uses the attention map to capture bilinear interactions. The approach is illustrated in \fig~\ref{fig:babe}.

\subsection*{Model Definition}

\textbf{Bimodal Embeddings} Let us denote the visual objects obtained from bottom-up attention mechanism\rs{CITE} by $\mathbf{V} \in \mathbb{R}^{o \times v}$, where $o$ is the number of visual objects and $v$ is the dimensionality of visual feature. The model embeds each question word into a 300 dimensional GloVe embedding\rs{CITE} and uses a Gated Recurrent Unit (GRU) to generate single vector representing the entire question: $\mathbf{Q}$. Our algorithm applies early fusion between visual and question features by concatenating each visual object with the question. The combined features are passed through multiple fully connected layers (FC) to generate Bimodal Embeddings $E = FC(V \oplus Q)$, where $\oplus$ denotes concatenation. 


\textbf{Attention Maps} Next, BARN uses bilinear attention mechanism\rs{CITE}, to predict multi-glimpse attention maps between bimodal embeddings $E$, where the attention map for $g^{th}$ glimpse is given by:
\begin{align}
A_g = softmax(((\mathbbm{1}.p_g ^ T) \circ E M) (E N)^T) \in \mathbb{R}^{o \times o}
\end{align}
Here, $M, N \in \mathbb{R}^{v \times d}$ are learnable parameters that reduce the dimension of each channel in $E$ into a $d$-dimensional vector. The number of channels in $E$ is same as the number of visual objects $o$. $M$ and $N$ are shared between all the glimpses. Next, $p_g \in \mathbb{R}^{d}$ is used to create separate attention map for each glimpse. These glimpses are all computed parallely. Also, $\mathbbm{1} \in \mathbb{R}^o$ is a column vector of ones, used to replicate $p_g^T$ rowwise and $\circ$ denotes Hadamard product. The values in the attention map can be interpreted as the relevance of corresponding embedding pair to answer the question. 

\textbf{Bilinear Interactions} We use the mechanism introduced in\rs{CITE} to capture bilinear interactions between bimodal embeddings. Let us denote the output of $g^{th}$ glimpse by: 
\begin{align}
    B_{g} = BAN(E, H_g, A_g).
\end{align}
Here, $H_g$ is the input for the $g^{th}$ glimpse. For the first glimpse, the input is simply the embedding itself i.e., $H_1 = E$. The $k^{th}$ element of $B_g$ is computed by taking attention-weighted sum over all embeddings:
\begin{align}
    B_{g,k} = \sum_{i=1}^o \sum_{j=1}^o (E_i M_k) A_{1,i,j} (H_{g,j} N_k)^T
\end{align}
where, $M_k$ and $N_k$ are the $k^{th}$ columns of learnable weights. 

\textbf{Residual Connections}
Following \rs{CITE}, we use residual connections to integrate information from multiple glimpses. To get the input for $(g+1)^{th}$ glimpse, we add the output from $g^{th}$ glimpse: $B_g$ to $H_g$: $H_{g+1} = H_g + B_g$. Of course the output of $(g+1)^th$ is given by the same formulation:
\begin{align}
B_{g+1} = BAN(E, H_{g+1})
\end{align}

\textbf{Answer Prediction} Finally, we pass $B_{G}$ through 1 fully connected layer to predict the answer, where $G$ is the total number of glimpses.

%Note that, Bilinear Attention Networks\rs{CITE} use same mechanism to capture bilinear interactions between visual objects and question words, which worked really well for natural VQA datasets, but did not enable compositional reasoning. Here we are using bimodal embeddings which are known to work for reasoning tasks. Hopefully, BARN will capture all the query-relevant visual and relational features required to answer questions in both natural and compositional reasoning VQA datasets.


\section{Experiments}
To make comparisons fair, we use same visual features in all experiments.

\subsection{Visual Features} 
We use bottom-up object proposals from pre-trained FasterRCNN~\cite{girshick2015fast} as our visual features. For natural images, we use FasterRCNN trained for object recognition, attribute recognition and bounding box regression on Visual Genome~\cite{krishna2017visual}. For CLEVR, we train a separate FasterRCNN for multi-class classification and bounding box regression. Each CLEVR object is associated with one of 8 colors (red, green, blue, purple, gray, brown, cyan, yellow), 3 shapes (sphere, cylinder, cube), 2 sizes (small, large) and 2 materials (shiny, matte). We label each CLEVR object as: $\textit{color\_shape\_size\_material}$, getting a total of 96 classes for multi-class classification. CLEVR dataset does not provide ground truth bounding boxes for regression, so, we estimate the bounding boxes by projecting the 3D objects from the scene annotations. We do not use attribute classification for CLEVR because class labels already identify the attributes. The feature length is 2048.

\textbf{Spatial Information} To encode position and size of an object, we append a flattened grid of (x, y) coordinates to visual features of the object. Specifically, we divide each bounding box into 16X16 grid of coordinates, with coordinates taken relative to the whole image. The coordinates are normalized to [0, 1] by dividing by image width and height. These numbers are concatenated with bottom-up features, obtaining a 2560 dimensional visual vector.

\subsection{Metrics}
\textbf{\gls{VQAv1} and \gls{VQAv2}} provide multiple answers per question, so we use the standard ``10-choose-3 VQA metric'':
\begin{align*}
acc(ans) = min(\frac{\text{number of times ``ans'' is chosen}}{3}, 1)
\end{align*}

For \textbf{\gls{TDIUC}}, we use the arithmetic and harmonic means over all question types: Arithmetic Mean Per Type (AMPT) and Harmonic Mean  Per Type (HMPT). AMPT is a better indicator of task generalization than simple accuracy and HMPT is skewed towards lowest performing tasks. 

We further use normalized metrics: Normalized AMPT (N-AMPT) and Normalized HMPT (N-HMPT) that test account for the imbalance in answer distribution. Normalized metrics are computed by first calculating accuracy for each unique answer for each question type and averaging them within each question type. Then, we take \textbf{Rest of the datasets} provide single answer to each question \rs{VERIFY This}, so we use simple accuracies for them.
arithmetic and harmonic means over all question types to obtain 
N-AMPT and N-HMPT. Difference between unnormalized and normalized metrics indicate lack of generalization to rare answers.

\textbf{Rest of the datasets} provide single answer to each question \rs{VERIFY This}, so we use simple accuracies for them.
\begin{table*}[htbp]
\centering
\begin{tabular}{lrrrrrr|r}
\hline
 Dataset/Algorithm & \multicolumn{1}{l}{UpDn} & \multicolumn{1}{l}{\qcg} & \multicolumn{1}{l}{BAN} & \multicolumn{1}{l}{MAC} & \multicolumn{1}{l}{RN} & \multicolumn{1}{l}{BRAN} & \multicolumn{1}{|l}{\# Questions}\\ \hline
Scene Recognition & 94.17 & 77.52 & \textbf{94.61} & 91.90 &  & & 66,706 \\
Sentiment Understanding & 62.93 & 56.23 & 65.01 & 67.25 &  & & 2,095 \\
Sport Recognition & 95.49 & 95.34 & 96.40 & 93.20 &  &  & 31,644 \\
Activity Recognition & 56.82 & 54.32 & 61.33 & 49.03 &  &   & 8,530 \\
Object Recognition & 88.28 & 88.14 & 89.18 & 84.67 &  &  & 93,555 \\
Object Presence & 95.63 & 95.71 & 96.16 & 93.76 &  &  & 657,134 \\
Positional Reasoning & 36.49 & 34.10 & 38.43 & 30.83 &  &  & 38,326 \\
Counting & 56.34 & 56.56 & 61.29 & 50.72 &  &  & 164,762 \\
Object Attributes & 56.92 & 55.80 & 59.31 & 51.26 &  &  & 28,676 \\
Color Attributes & 72.21 & 49.35 & 73.36 & 63.13 &  &  & 195,564 \\
Utility Affordance & 30.24 & 33.33 & 33.95 & 29.62 &  & & 521 \\
Absurd & 80.29 & 91.60 & 84.20 & 91.79 &  & & 366,654 \\ \hline
Overall (Arithmetic MPT) & 68.82 & 65.67 & 71.10 & 66.43 &  &  \\
Overall (Harmonic MPT) & 60.47 & 57.84 & 63.69 & 56.74 &  &  \\ \hline
Overall (Arithmetic N-MPT) & 38.93 & 37.43 & 40.65 & 39.02 &  &  \\
Overall (Harmonic N-MPT) & 21.27 & 19.81 & 22.64 & 21.44 &  &  \\ \hline
Simple Accuracy & 82.91 & 82.05 & 84.81 & 82.53 &  &  \\ \hline
\end{tabular}
\caption{Comparison of VQA models on the 12 task types present in TDIUC. The table shows simple accuracy for each task type and both normalized and unnormalized formulations of arithmetic and harmonic mean per type accuracy (MPT) indicating overall performance.}
\label{tbl:tdiuc}
\end{table*}



\section{Results}
\subsection{Evaluation of Natural Image Understanding with VQA1 and VQA2}
\tbl~\ref{tbl:all_vs_all} shows the performance of all VQA algorithms on VQA1 and VQA2. Natural VQA algorithms outperform MAC and RN on VQA1 and VQA2, with BAN standing out as the clear winner. BAN outperforms next best models by significant margins of 4.68\% on VQA1 and 3.89\% on VQA2. UpDn and \qcg achieve comparable performances (within 2\% of each other) on all natural VQA datasets. RN ... MAC performs significantly worse than RN on VQA2, probably because MAC does not have a direct interaction between question and visual features, rather they interact indirectly through an attention mechanism. Of course, these performances may be because natural VQA algorithms exploit biases much better than MAC. However, just because MAC does not exploit biases does not mean it is capable of natural concept understanding, as indicated by the performance drops on CVQA and VQACP.

\subsection{Testing Concept Composition with \cvqa}
As presented in \tbl~\ref{tbl:cvqa_and_vqacp},  accuracies on CVQA are lower than VQA1, indicating that all algorithms struggle when asked to combine concepts in new ways. Even natural algorithms have significant overall performance drop (5-8 \%), indicating a lack of concept understanding. Performance drop for MAC is even more pronounced at 20\%, showing that its compositional reasoning mechanism is not adequate for combine natural concepts.
\begin{table}
\begin{tabular}{cccccc}
\hline
& & Y/N & Number & Other & Overall \\
\hline
\multirow{3}{*}{ UpDn } & VQA1 & 80.06 & 35.63 & 66.33 & 66.80 \\
& CVQA & 70.62 & 22.30 & 58.70 & 60.94 \\
& VQACP & 36.16 & 11.21 & 39.78 & 39.00 \\
\hline
\multirow{3}{*}{ \qcg } & VQA1 & 81.70 & 42.19 & 65.46 & 65.94 \\
& CVQA & 60.11 & 21.97 & 64.73 & 60.67 \\
& VQACP & 47.21 & 18.30 & 38.79 & 37.87 \\
\hline
\multirow{3}{*}{ BAN } & VQA1 & 82.40 & 43.17 & 69.57 & 71.48 \\
& CVQA & 74.06 & 28.11 & 62.12 & 63.40 \\
& VQACP & 39.56 & 11.51 & 42.80 & 42.04 \\
\hline
\multirow{3}{*}{ MAC } & VQA1 & 76.79 & 29.87 & 60.02 & 63.88 \\
& CVQA & 71.02 & 20.28 & 51.60 & 43.56 \\
& VQACP & 35.20 & 11.38 & 35.97 & 33.86 \\
\hline
\multirow{3}{*}{ RN } & VQA1 & N/A & N/A & N/A & N/A \\
& CVQA & N/A & N/A & N/A & N/A \\
& VQACP & 34.50 & 11.65 & 36.64 & 36.30 \\
\hline
\multirow{3}{*}{ BRAN } & VQA1 & N/A & N/A & N/A & N/A \\
& CVQA & N/A & N/A & N/A & N/A \\
& VQACP & N/A & N/A & N/A & N/A \\
\hline
\end{tabular}
\caption{Considering VQA1 as the benchmark, all VQA algorithms struggle to generalize to unseen concept compositions (CVQA), and even more severely to different answer distributions (VQACP).}
\label{tbl:cvqa_and_vqacp}
\end{table}

\begin{table*}
\centering
\begin{tabular}{lrrrrrr}
\hline
& UpDn & \qcg & BAN & MAC & RN & BRAN \\
\hline
Count & 55.83 & 41.38 & 79.54 & 95.46 & 90.90 & \\
Exist & 73.52 & 62.62 & 87.52 & 99.18 & 98.40 & \\
Compare Numbers & 62.30 & 58.40 & 68.08 & 93.27 & 84.99 & \\
Query Attribute & 68.96 & 30.16 & 70.68 & 99.59 & 98.19 & \\
Compare Attribute & 62.38 & 50.69 & 73.82 & 99.33 & 97.81 & \\
\hline
\end{tabular}
\caption{Performance of VQA algorithms on 5 different CLEVR query types. Natural VQA algorithms struggle on all CLEVR question types.}
\label{tbl:clevr_per_type}
\end{table*}
\subsection{Evaluation on New Answer Distributions with \vqacp}
By comparing the performances on VQA1 and VQACP as presented in \tbl~\ref{tbl:cvqa_and_vqacp}, we can see that all VQA algorithms exhibit a large performance drop when tested under new answer distributions. While BAN outperforms every other model on natural VQA datasets, it also exhibits the largest drop in performance of 8\% from VQA1 to VQACP, among the natural VQA algorithms. The results indicate that neither natural algorithms nor compositional algorithms are capable of true concept understanding and rather base their answers on statistical biases.

\subsection{Evaluation of Nuanced Task Understanding with TDIUC}
Since the number of questions per task significantly differ based on the task type, we take question count into account when making comparisons on TDIUC. As presented in \tbl~\ref{tbl:tdiuc}, all algorithms perform well on tasks with numerous examples in the dataset: sport recognition ($>$ 31K questions), object presence ($>$ 657K questions) and scene recognition ($>$66K questions) and perform poorly when there are only  a few examples: activity recognition (8.5K questions), sentiment understanding (2K questions) and utility/affordance (531 questions). Positional reasoning and counting are the most challenging tasks, and algorithms struggle with them even though there are a large number of questions (38K and 164K respectively) for both tasks.

\textbf{TDIUC Results with Unbiased Metrics} While each method achieves a simple accuracy $>82\%$, the AMPT scores are below 72\%. This discrepancy between simple accuracy and AMPT metric indicates that the algorithms struggle to generalize to multiple tasks. As proposed in\rs{CITE}, Normalized Arithmetic Mean Per Type (N-AMPT) provides a measure of generalization to rare answers because it takes answer frequency into account. N-AMPT is computed by taking accuracies of unique answers within a task, averaging them for each task and then computing the mean over all task types. N-AMPT scores are 27 - 30\% lower than unnormalized MPT scores, indicating that the algorithms struggle with rare answers.

\subsection{Test of Compositional Reasoning Skills with CLEVR}
\tbl~\ref{tbl:clevr_per_type} clearly shows that natural VQA algorithms do not possess compositional reasoning skills. BAN achieves an overall score of 75.56\% on CLEVR, which is the highest for natural VQA algorithm, but it is still 20\% below relation networks. \qcg~represents the entire scene as a graph and captures interactions between all visual objects, however it performs disastrously on CLEVR, achieving only 43.51\%. We think the problem with \qcg's weight parameterization, which is based only spatial coordinates and a attention score from adjacency matrix. Such weights do not encode information visual relationships required to compare visual properties of objects.
